Synthetic Gaia DR3 surveys from the FIRE cosmological simulations of Milky-Way-mass galaxies

The third data release (DR3) of Gaia has provided a five-fold increase in the number of radial velocity measurements of stars, as well as a stark improvement in parallax and proper motion measurements. To help with studies that seek to test models and interpret Gaia DR3, we present nine Gaia synthetic surveys, based on three solar positions in three Milky-Way-mass galaxies of the Latte suite of the Fire-2 cosmological simulations. These synthetic surveys match the selection function, radial velocity measurements, and photometry of Gaia DR3, adapting the code base Ananke, previously used to match the Gaia DR2 release in Sanderson et al. 2020. The synthetic surveys are publicly available and can be found at http://ananke.hub.yt/. Similarly to the previous release of Ananke, these surveys are based on cosmological simulations and thus able to model non-equilibrium dynamical effects, making them a useful tool in testing and interpreting Gaia DR3.

==> tables/tab_data_model_notdeluxe.tex <==
%\begin{turnpage}
\begin{table*}
\caption{Data Model for Synthetic Surveys}
\label{tab:data_model}
\begin{tabular}{lp{8cm}cc}
\hline
Quantity &
Explanation & 
Data Type & 
Unit
\\
\hline
\multicolumn{4}{c}{\textit{Fields with names identical to those in DR2}} \\
\hline
\multicolumn{4}{c}{Indices} \\
\hline
\texttt{random\_index} & Random index used to select subsets & long & \nodata \\
\hline
\multicolumn{4}{c}{Astrometry} \\
\hline
\texttt{ra} & Right ascension & double & Angle (deg) \\
\texttt{ra\_error} & Standard error of R.A. & double & Angle (deg) \\
\texttt{dec} & decl. & double & Angle (deg) \\
\texttt{dec\_error} & Standard error of decl. & double & Angle (deg) \\
\texttt{parallax} & Parallax & double & Angle (mas) \\
\texttt{parallax\_error} & Standard error of parallax & double & Angle (mas) \\
\texttt{parallax\_over\_error} & Parallax divided by its error & float & \nodata \\
\texttt{pmra} & Proper motion in R.A. direction & double & Angular Velocity (\masyr) \\
\texttt{pmra\_error} & Standard error of proper motion in R.A. direction & double & Angular Velocity (\masyr) \\
\texttt{pmdec} & Proper motion in decl. direction & double & Angular Velocity (\masyr) \\
\texttt{pmdec\_error} & Standard error of proper motion in decl. direction & double & Angular Velocity (\masyr) \\
\texttt{l} & Galactic longitude (converted from R.A., decl.) & double & Angle (deg) \\
\texttt{b} & Galactic latitude (converted from R.A., decl.) & double & Angle (deg) \\
\hline
\multicolumn{4}{c}{Photometry} \\
\hline
\texttt{phot\_g\_mean\_mag} & Extincted apparent $G$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_bp\_mean\_mag} & Extincted apparent $G_{BP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_rp\_mean\_mag} & Extincted apparent $G_{RP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{bp\_rp} & Reddened $G_{BP}-G_{RP}$ color & float & Magnitude (mag) \\
\texttt{bp\_g} & Reddened $G_{BP}-G$ color & float & Magnitude (mag) \\
\texttt{g\_rp} & Reddened $G-G_{RP}$ color & float & Magnitude (mag) \\
\hline
\multicolumn{4}{c}{Spectroscopy} \\
\hline
\texttt{radial\_velocity} & Radial velocity & double & Velocity (\kmsec) \\
\texttt{radial\_velocity\_error} & Standard error of radial velocity & double & Velocity (\kmsec) \\
\hline
\multicolumn{4}{c}{\textit{Other fields not in the Gaia DR2 data model}} \\
\hline
\multicolumn{4}{c}{Indices} \\
\hline
\texttt{starid} & array index of the star (per mock catalog) & long & \nodata \\
\texttt{parentid} & array index of the generating star particle in the snapshot file & long & \nodata \\
\texttt{partid} & 0 if phase-space coordinates are identical to the generating star particle, 1 otherwise & short & \nodata \\
\hline
\multicolumn{4}{c}{Phase Space} \\
\hline
\texttt{ra\_true} & true R.A. & double & Angle (deg) \\
\texttt{dec\_true} & true decl. & double & Angle (deg) \\
\texttt{dmod\_true} & true distance modulus & double & Magnitude (mag) \\
\texttt{ra\_cosdec\_error} & standard error in R.A.$\cos{(\rm decl.)}$ & double & Magnitude (deg) \\
\texttt{parallax\_true} & true parallax & double & Angle (mas) \\
\texttt{pmra\_true} & true pm in R.A. direction & double & Angular Velocity (\masyr) \\
\texttt{pmdec\_true} & true pm in decl. direction & double & Angular Velocity (\masyr) \\
\texttt{radial\_velocity\_true} & true RV & double & Velocity (\kmsec) \\
\texttt{l\_true} & true Galactic long & double & Angle (deg) \\
\texttt{b\_true} & true Galactic lat & double & Angle (deg) \\
\texttt{pml} & pm in Galactic long direction & double & Angular Velocity (\masyr) \\
\texttt{pmb} & pm in Galactic lat direction & double & Angular Velocity (\masyr) \\
\texttt{pml\_true} & true pm in Galactic long direction & double & Angular Velocity (\masyr) \\
\texttt{pmb\_true} & true pm in Galactic lat direction & double & Angular Velocity (\masyr) \\
\texttt{px\_true, py\_true, pz\_true} & true position relative to LSR & double & Distance (kpc) \\
\texttt{vx\_true, vy\_true, vz\_true} & true velocity relative to LSR & double & Velocity (\kmsec) \\
\hline
\multicolumn{4}{c}{Photometry} \\
\hline
\texttt{phot\_g\_mean\_mag\_true} & true (i.e., after extinction, but before error convolution) apparent $G$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_bp\_mean\_mag\_true} & true apparent $G_{BP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_rp\_mean\_mag\_true} & true apparent $G_{RP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_g\_mean\_mag\_int} & intrinsic (i.e., before extinction or error convolution) apparent $G$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_bp\_mean\_mag\_int} & intrinsic apparent $G_{BP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_rp\_mean\_mag\_int} & intrinsic apparent $G_{RP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_g\_mean\_mag\_abs} & absolute $G$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_bp\_mean\_mag\_abs} & absolute $G_{BP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_rp\_mean\_mag\_abs} & absolute $G_{RP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_g\_mean\_mag\_error} & Standard error of $G$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_bp\_mean\_mag\_error} & Standard error of $G_{BP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{phot\_rp\_mean\_mag\_error} & Standard error of $G_{RP}$-band mean magnitude & float & Magnitude (mag) \\
\texttt{bp\_rp\_true} & true $G_{BP}-G_{RP}$ color & float & Magnitude (mag) \\
\texttt{bp\_g\_true} & true $G_{BP}-G$ color & float & Magnitude (mag) \\
\texttt{g\_rp\_true} & true $G-G_{RP}$ color & float & Magnitude (mag) \\
\texttt{vmini\_true} & true $V-I$ color used for error modeling & float & Magnitude (mag) \\
\hline
\multicolumn{4}{c}{Extinction} \\
\hline
\texttt{lognh} & $\log_{10}$ equivalent H column density along line of sight to star & float & surface number density(cm$^{\rm -2}$) \\
\texttt{ebv} & $E(B-V)$ reddening, calculated from $N_{\rm H}^{eff}$ & float & Magnitude (mag) \\
\texttt{A0} & $A_0$, extinction at 550\,nm, assuming $R_V = 3.1$ & float & Magnitude (mag) \\
\texttt{a\_g\_val} & true line-of-sight extinction in the $G$ band, $A_G$ & float & Magnitude (mag) \\
\texttt{e\_bp\_min\_rp\_val} & true line-of-sight reddening $G_{BP}-G_{RP}$ & float & Magnitude (mag) \\
\hline
\multicolumn{4}{c}{Spectroscopy} \\
\hline
\texttt{radial\_velocity\_error\_corr\_factor} & correction factor for \texttt{radial\_velocity\_error} & double & Velocity (\kmsec) \\
\hline
\multicolumn{4}{c}{Stellar Parameter} \\
\hline
\texttt{mact} & current stellar mass & float & Mass (Solar Mass) \\
\texttt{mtip} & mass of a star at tip of giant branch for given age, metallicity & float & Mass (Solar Mass) \\
\texttt{mini} & stellar mass on zero-age main sequence & float & Mass (Solar Mass) \\
\texttt{age} & $\log_{10}$ of stellar age; identical for all stars generated from the same particle & float & Time (log yr) \\
\texttt{teff} & stellar effective temperature & float & Temperature (K) \\
\texttt{logg} & surface gravity & float & Surface Gravity (log cgs) \\
\texttt{lum} & $\log_{10}$ of stellar luminosity & float &  Luminosity (log Solar Luminosity) \\
\hline
\multicolumn{4}{c}{Abundances} \\
\hline
\texttt{feh} & [Fe/H] & float & Magnitude (mag) \\
\texttt{alpha} & [Mg/Fe] & float & Magnitude (mag) \\
\texttt{carbon} & [C/H] & float & Magnitude (mag) \\
\texttt{helium} & [He/H] & float & Magnitude (mag) \\
\texttt{nitrogen} & [N/H] & float & Magnitude (mag) \\
\texttt{sulphur} & [S/H] & float & Magnitude (mag) \\
\texttt{oxygen} & [O/H] & float & Magnitude (mag) \\
\texttt{silicon} & [Si/H] & float & Magnitude (mag) \\
\texttt{calcium} & [Ca/H] & float & Magnitude (mag) \\
\texttt{magnesium} & [Mg/H] & float & Magnitude (mag) \\
\texttt{neon} & [Ne/H] & float & Magnitude (mag) \\
\hline
\multicolumn{4}{c}{Selection Function} \\
\hline
\texttt{n\_transit} & number of expected transits & long & \nodata \\
\texttt{prob\_ruwe1p4} & probability of being selected with good astrometry & float & \nodata \\
\texttt{prob\_rvs} & probability of being selected with RV measurement & float & \nodata \\
\texttt{selected\_ruwe1p4} & flag if the star is selected with good astrometry & boolean & \nodata \\
\texttt{selected\_rvs} & flag if the star is selected with RV measurement & boolean & \nodata \\
\hline
\multicolumn{4}{c}{Quality Control} \\
\hline
\texttt{flags} & bitmask flag for quality control; see Section~\ref{sec:flags} & long & \nodata \\
\hline
\end{tabular}
\end{table*}
%\end{turnpage}

==> tables/tab_photo_error_coeff.tex <==
\begin{table}
\caption{Coefficients of the photometric errors in Eq.~\ref{eq:photo_error}.}
\label{tab:photo_error_coeff}
\centering
\begin{tabular}{cccccc}
\hline
\hline
\multicolumn{1}{l}{}                     &     &             & $V-I$       & $(V-I)^2$  & $(V-I)^3$   \\ \hline
\multicolumn{1}{l}{\multirow{3}{*}{$G$}} & $a$ & $-1.310247$ &             &            &             \\
\multicolumn{1}{l}{}                     & $b$ & $0.2702828$ &             &            &             \\
\multicolumn{1}{l}{}                     & $c$ & $-3.702239$ &             &            &             \\ \hline
\multirow{3}{*}{$G_{BP}$}                & $a$ & $1.043270$  & $0.355123$  & $0.044390$ & $-0.000562$ \\
                                         & $b$ & $1.465592$  & $0.195768$  & $0.018878$ & $-0.000400$ \\
                                         & $c$ & $-1.866968$ & $-0.205807$ & $0.060769$ & $0.0002620$  \\ \hline
\multirow{3}{*}{$G_{RP}$}                & $a$ & $1.615927$  & $-0.636628$ & $0.114126$ & $-0.007597$ \\
                                         & $b$ & $1.783906$  & $-0.318499$ & $0.057112$ & $-0.003803$ \\
                                         & $c$ & $-3.042268$ & $-0.091569$ & $0.027352$ & $-0.001923$ \\
\hline
% \hline
\end{tabular}
\end{table}
